Long-Lived Particles at the Energy Frontier: The MATHUSLA Physics Case

We examine the theoretical motivations for long-lived particle (LLP) signals at the LHC in a comprehensive survey of Standard Model (SM) extensions. LLPs are a common prediction of a wide range of theories that address unsolved fundamental mysteries such as naturalness, dark matter, baryogenesis and neutrino masses, and represent a natural and generic possibility for physics beyond the SM (BSM). In most cases the LLP lifetime can be treated as a free parameter from the $\mu$m scale up to the Big Bang Nucleosynthesis limit of $\sim 10^7$m. Neutral LLPs with lifetimes above $\sim$ 100m are particularly difficult to probe, as the sensitivity of the LHC main detectors is limited by challenging backgrounds, triggers, and small acceptances. MATHUSLA is a proposal for a minimally instrumented, large-volume surface detector near ATLAS or CMS. It would search for neutral LLPs produced in HL-LHC collisions by reconstructing displaced vertices (DVs) in a low-background environment, extending the sensitivity of the main detectors by orders of magnitude in the long-lifetime regime. In this white paper we study the LLP physics opportunities afforded by a MATHUSLA-like detector at the HL-LHC. We develop a model-independent approach to describe the sensitivity of MATHUSLA to BSM LLP signals, and compare it to DV and missing energy searches at ATLAS or CMS. We then explore the BSM motivations for LLPs in considerable detail, presenting a large number of new sensitivity studies. While our discussion is especially oriented towards the long-lifetime regime at MATHUSLA, this survey underlines the importance of a varied LLP search program at the LHC in general. By synthesizing these results into a general discussion of the top-down and bottom-up motivations for LLP searches, it is our aim to demonstrate the exceptional strength and breadth of the physics case for the construction of the MATHUSLA detector.

==> _tmp_ <==
\author{
Editors: \\
R.~Contino$^{1,2}$,\, 
D.~Curtin$^{3}$,\,
A.~Katz$^{1,4}$,\,
M.~L.~Mangano$^{1}$,\,
G.~Panico$^{5}$,\,
M.~J.~Ramsey-Musolf$^{6,7}$,\, 
G.~Zanderighi$^{1}$\,
\\
Contributors: \\
C.~Anastasiou$^{8}$,\,
W.~Astill$^{9}$,\,
J.~K.~Behr$^{10,11}$,\,
W.~Bizon$^{9}$,\,
P.~S.~Bhupal~Dev$^{12}$,\,
D.~Bortoletto$^{10}$,\,
F.~Caola$^{1}$,\,
J.~Chakrabortty$^{13}$,\,
C.-Y.~Chen$^{14,15,16}$,\,
F.~Dulat$^{8}$,\,
G.~Bambhaniya$^{17}$,\,
D.~Buttazzo$^{18}$
D.~de~Florian$^{19}$,\,
C.~Englert$^{20}$,\,
J.~A.~Frost$^{10}$,\,
B.~Fuks$^{21}$,\,
T.~Gherghetta$^{22}$,\,
G.~Giudice$^{1}$,\,
J.~Gluza$^{23}$,\,
N.~Greiner$^{24}$,\,
H.~Gray$^{25}$,\,
N.~P.~Hartland$^{10}$,\,
C.~Issever$^{10}$,\,
T.~Jeli\'nski$^{23}$,\,
A.~Karlberg$^{9}$,\,
J.~H.~Kim,$^{26,27,28}$,\,
F.~Kling$^{29}$,\,
A.~Lazopoulos$^{8}$,\,
S.~J.~Lee$^{30,31}$,\,
G.~Luisoni$^{1}$,\,
J.~Mazzitelli$^{19,32}$,\,
B.~Mistlberger$^{1}$,\,
P.~Monni$^{9}$,\,
K.~Nikolopoulos$^{33}$,\,
R.~N~Mohapatra$^{3}$,\,
A.~Papaefstathiou$^{1}$,\,
M.~Perelstein$^{34}$,\,
F.~Petriello$^{35}$,\,
T.~Plehn$^{36}$,\,
P.~Reimitz$^{36}$,\,
J.~Ren$^{37}$,\,
J.~Rojo$^{10}$,\,
K.~Sakurai$^{38}$,\,
T.~Schell$^{36}$,\,
F.~Sala$^{39}$,\,
M.~Selvaggi$^{40}$,\,
H.-S.~Shao$^{1}$,\,
M.~Son$^{26}$,\,
M.~Spannowsky$^{38}$,\,
T. Srivastava$^{13}$,\,
S.-F.~Su$^{29}$,\,
R. Szafron$^{41}$,\,
T.~Tait$^{42}$,\,
A.~Tesi$^{43}$,\,
A.~Thamm$^{44}$,\,
P.~Torrielli$^{45}$,\,
F.~Tramontano$^{46}$,\,
J.~Winter$^{47}$,\,
A.~Wulzer$^{48}$,\,
Q.-S.~Yan$^{49,50,51}$,\,
W.~M.~Yao$^{52}$,\,
Y.-C.~Zhang$^{53}$,\,
X.~Zhao$^{49}$,\,
Z.~Zhao$^{49,54}$,\,
Y.-M.~Zhong$^{55}$,\, 
Q.-H.~Cao$^{50,56,57}$,\, 
S.-L.~Chen$^{50,58}$,\, 
Y.~Liu$^{56}$
\vspace*{2cm}
}

\institute{
$^{1}$ CERN, TH Department, CH-1211 Geneva, Switzerland. \\
$^{2}$ EPFL, Lausanne, Switzerland. \\
$^{3}$Maryland Center for Fundamental Physics, Department of Physics, University of Maryland, College
Park, MD 20742, USA\\
$^{4}$Universit\'{e} de Gen\`{e}ve, Department of Theoretical Physics and Center for Astroparticle Physics,
24 quai E. Ansermet, CH-1211, Geneva 4, Switzerland\\
$^{5}$ IFAE, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Barcelona\\
$^{6}$ Amherst Center for Fundamental Interactions, Physics Department,University of Massachusetts Amherst, Amherst, MA 01003, USA\\
$^{7}$ Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, CA 91125 USA\\
$^{8}$  Institute for Theoretical Physics, ETH Z\"urich,  8093 Z\"urich, Switzerland \\
$^{9}$ Rudolf Peierls Centre for Theoretical Physics, 1 Keble Road, University of Oxford, UK \\
$^{10}$ Physics Department, 1 Keble Road, University of Oxford, United Kingdom\\
$^{11}$ Deutsches Elektronen-Synchrotron (DESY), Notkestrasse 85, D-22607 Hamburg, Germany\\
$^{12}$Max-Planck-Institut f\"ur Kernphysik, Saupfercheckweg 1,
D-69117 Heidelberg, Germany\\
$^{13}$  Department of Physics, Indian Institute of Technology, Kanpur-208016, India\\
$^{14}$ Department of Physics, Brookhaven National Laboratory, Upton, New York 11973, USA\\
$^{15}$ Department of Physics and Astronomy, University of Victoria, Victoria, British Columbia V8P 5C2, Canada\\
$^{16}$ Perimeter Institute for Theoretical Physics, Waterloo, Ontario N2J 2W9, Canada\\
$^{17}$ Theoretical Physics Division, Physical Research Laboratory, Ahmedabad-380009, India\\
$^{18}$ Physik-Institut, Universit\"at Z\"urich, CH-8057 Z\"urich, Switzerland \\ 
$^{19}$ International Center for Advanced Studies (ICAS), UNSAM, Campus Miguelete, 25 de Mayo y Francia, (1650) Buenos Aires, Argentina\\
$^{20}$ SUPA, School of Physics and Astronomy, University of Glasgow,
Glasgow G12 8QQ, UK \\
$^{21}$ Sorbonne Universit\'es, UPMC Univ.~Paris 06, UMR 7589, LPTHE, F-75005 Paris, France.  CNRS, UMR 7589, LPTHE, F-75005 Paris, France \\
$^{22}$ School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA\\
 $^{23}$ Institute of Physics, University of Silesia, Uniwersytecka 4, 40-007 Katowice, Poland\\
$^{24}$ Physik Institut, Universit\"at Z\"urich, Winterthurerstrasse 190, CH-8057 Z\"urich, Switzerland \\
$^{25}$ CERN, EP Department, CH-1211 Geneva, Switzerland. \\
$^{26}$ Department of Physics, Korea Advanced Institute of Science and Technology, 335 Gwahak-ro, Yuseong-gu, Daejeon 305-701, Korea \\
$^{27}$ Center for Theoretical Physics of the Universe, IBS, 34051 Daejeon, Korea\\
$^{28}$ Center for Axion and Precision Physics Research, IBS, 34141 Daejeon, Korea \\
$^{29}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{30}$ Department of Physics, Korea University, Seoul 136-713, Korea\\
$^{31}$ School of Physics, Korea Institute for Advanced Study, Seoul 130-722, Korea\\
$^{32}$ Departamento de Fisica and IFIBA, FCEyN, Universidad de
Buenos Aires, (1428) Pabellon 1 Ciudad Universitaria, Capital Federal,
Argentina \\
$^{33}$ School of Physics and Astronomy, University of Birmingham,
Birmingham, B15 2TT, United Kingdom \\
$^{34}$Laboratory for Elementary Particle Physics, Cornell University,
Ithaca, NY 14853, USA\\
$^{35}$ 
Northwestern University, Department of Physics and Astronomy, 2145
Sheridan Road, 
Evanston, Illinois 60208-3112, USA\\
$^{36}$ Institut f\"ur Theoretische Physik, Universit\"at Heidelberg, Germany \\
$^{37}$ Department of Physics, University of Toronto, Toronto, Ontario, Canada M5S1A7\\
$^{38}$ IPPP, Department of Physics, University of Durham, Science Laboratories, South Road, Durham, DH1 3LE, UK\\
$^{39}$ 2LPTHE, CNRS, UMR 7589, 4 Place Jussieu, F-75252, Paris, France\\
$^{40}$ Centre for Cosmology, Particle Physics and Phenomenology CP3, Universit\'e Catholique de Louvain, Chemin du Cyclotron, 1348 Louvain la Neuve, Belgium\\
$^{41}$ Department of Physics, University of Alberta, Edmonton, AB
T6G 2E1, Canada\\
$^{42}$ Department of Physics and Astronomy, University of California, Irvine, CA 92697, USA\\
$^{43}$ Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA\\
$^{44}$ PRISMA Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany\\
$^{45}$ Dipartimento di Fisica, Universit\`a di Torino, and INFN, Sezione di Torino, \\
Via P.~Giuria~1, I-10125, Turin, Italy \\
$^{46}$ Universit\`a di Napoli ``Federico II'' and INFN, Sezione di
Napoli, 80126 Napoli, Italy \\
$^{47}$Department of Physics and Astronomy, Michigan State University,
East Lansing, MI 48824, USA\\
$^{48}$Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova and
INFN, Sezione di Padova, via Marzolo 8, I-35131 Padova, Italy\\
$^{49}$ School of Physical Sciences, University of Chinese Academy of Sciences, Beijing 100049, P. R. China\\
$^{50}$ Center for High-Energy Physics, Peking University, Beijing 100871, P. R. China\\
$^{51}$ Center for future high energy physics, Chinese Academy of Sciences 100049, P. R. China\\
$^{52}$ Lawrence Berkeley National Lab (LBNL), One Cyclotron Rd, Berkeley, CA94720, USA\\
$^{53}$ Service de Physique Th\'eorique, Universit\'e Libre de Bruxelles, Boulevard du Triomphe, CP225, 1050 Brussels, Belgium\\
$^{54}$ Department of Physics, University of Siegen, 57068 Siegen, Germany\\
$^{55}$ C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, New York 11794, USA\\
$^{56}${Department of Physics and State Key Laboratory of Nuclear
Physics and Technology, Peking University, Beijing 100871, China} \\
$^{57}${Collaborative Innovation Center of Quantum Matter,
Beijing 100871, China} \\
$^{58}${Key Laboratory of Quark and Lepton Physics (MoE) and Institute of
Particle Physics, Central China Normal University, Wuhan 430079,
China} \\
}


==> section_decaychains.tex <==
%\newcommand{\sint}{s_{\theta}}
%\newcommand{\mphi}{m_{\phi}}

\subsection[Extended Decay Chains]{Extended Decay Chains\footnote{Thomas Flacke, Claudia~Frugiuele, Elina~Fuchs, Rick~S.~Gupta, Gilad~Perez and Matthias~Schlaffer}}
\label{sec:decaychains}


%\DC{abstract:}  We estimate the prospects of detecting a long-lived relaxion with the MATHUSLA detector. The minimal model of relaxion-Higgs mixing, requiring a relaxion mass above a GeV and a sufficient production rate, results in too prompt relaxion decays to reach MATHUSLA. Therefore we consider also a relaxion model with additional long-lived particles. Furthermore we propose to consider the detection feasibility of sub-GeV long-lived particles.

In \Sec{sec:relaxion} the detection prospects for a relaxion were considered.  In this section we consider a particular variant of relaxion model featuring additional long-lived particles.  This results in extended decay chain signatures that can be observed at MATHUSLA.

\subsubsection{Relaxion models with additional ultra long-lived BSM particles (ULLPs)}
A heavy relaxion could yield interesting signatures in MATHUSLA if the relaxion can also decay into ultra long-lived BSM particles (ULLPs) $X$. The presence of such particles in relaxion models has been proposed in \cite{Choi:2016kke} in order to solve a cosmological problem. Reheating can de-stabilize the electroweak vacuum established by the relaxion mechanism. The relaxion field starts to re-roll, and adding a coupling of the relaxion to an ULLP, which in  \cite{Choi:2016kke}  is chosen to be a dark photon, provides an additional friction term in the evolution equation of the relaxion which can stop the relaxion rolling after re-heating. \DC{can we elaborate on this very slightly? does the coupling have to be to ULLP or just any additional coupling?}

If such a ULLP is present and it is produced from relaxion decays, then its production cross-section is dictated by the relaxion production discussed in Ref.~\cite{Flacke:2016szy}, while its lifetime follows from the ULLP couplings to Standard Model particles. Realizations of scalar or dark photon ULLPs are possible to construct. \DC{section refs} In the following we give estimates of the number of events which could be measured in MATHULSA in a more general description, in terms of the branching ratios, life-times, and masses of the relaxion and the ULLP.

\vspace{4mm} \noindent \emph{Production from $B$-meson decays} \vspace{2mm}
%\label{sec:B2}
%this label is used nowhere
 \\GeV-scale relaxions can be produced in $B \to K \phi$ decays. The $b \bar{b}$ production cross-section at the LHC is around 500$\,\mu b$~\cite{Altarelli:2008xy}. This means that with 3\,$ab^{-1}$ integrated luminosity the number of $B$-mesons produced is,
\be
N_B= 5 \times 10^{14}.
\ee 
These $B$-mesons have a branching ratio given by
\be
Br(B\to K\phi)=s_\theta^2\times 0.5\times \frac{2 |p^{\rm rest}_\phi|}{m_B}\times F_K^2(m_\phi)\,,
\ee
where $s_\theta$ is the Higgs-relaxion mixing angle, $|p^{\rm rest}_\phi|$ is the magnitude of the relaxion momentum in the rest frame of the $B$-meson, and $F^2_K(m_\phi) = \left( 1- \frac{m^2_\phi}{38\gev^2}\right)^{-1}$~\cite{Clarke:2013aya}. The number of events that MATHUSLA can detect is given by
\be
N_{\rm events}\approx N_B \,Br(B\to K\phi) \,Br(\phi \to XX) \,{\cal G}_B  \,2 \,\tilde{f}_\tau
\label{eq:NBev2}
\ee
where ${\cal G}_B$ is a geometrical factor smaller than unity denoting the fraction of relaxions emitted in the direction of the MATHUSLA detector, and $\tilde{f}_\tau$ is the fraction of these events where the relaxion decays in the 20\,m thick MATHUSLA detector.  
We implicitly assume $m_\phi \ll 30$\,GeV (the typical momentum of the $B$ decay products) \DC{isn't this a given since $m_\phi < m_B$?} and $m_\phi > 2 m_X$. In this case, the relaxion is boosted along the direction of the original $B$, and the two $X$ resulting from the $\phi$ decay lie in a narrow cone around this direction.  The factor of $\sim 2$ arises because only one of the two $X$ particles which pass the detector need to decay in it in order to trigger the event.  The maximal value for $\tilde{f}_\tau$ is 
\be
\tilde{f}_\tau < \exp\left(\frac{-l}{\gamma \beta c \tau_X} \right)-\exp\left(-\frac{l+20/\sin \vartheta}{\gamma \beta c \tau_X}\right),
\ee
still with  $\sin \vartheta=0.32$, and a boost factor $\gamma \beta=|p_\phi|/ m_\phi$ where, $|p_\phi|$ corresponds to the magnitude of the momentum  of the decay products from $B$-decays.

%[Remark: In  Eq.~(\ref{eq:NBev2}), the  geometrical factor ${\cal G}_B$ can for now be estimated from the $\eta$ distribution in $b\bar{b}$ events in the regime $0.7 < \eta < 1.8$ corresponding to the currently assumed MATHUSLA geometry. ]

A current bound on $Br(B\to K\phi)\times Br(\phi \to XX)$ arrises from the bound on $Br(B \to K \nu\bar{\nu})\lesssim 1.4\times 10^{-5}$ (see Eq.(14) of Ref.~\cite{Clarke:2013aya} ). Thus, in production from $B$ decays, new physics will be tested if  $\,{\cal G}_B \,\tilde{f}_\tau \gtrsim (1.5\cdot10^{10})^{-1}$. \DC{just make this $\gtrsim 10^{-10}$?}


\vspace{4mm} \noindent \emph{Production from Higgs decays}  \vspace{2mm} \\
Higgs decays into relaxions with a subsequent decay $\phi \rightarrow XX$ provide another potential signal with 
\be
N_{\rm events}\approx N_h \,Br(h\to \phi\phi) \,Br(\phi \to XX) \,{\cal G}_h  \,2 \,\tilde{f}'_\tau.
\label{eq:NBev2h}
\ee
With $N_h = \mathcal{O}(10^{8})$, and an expected bound of $Br(h\rightarrow \rm{inv})\lesssim 0.1$ in the LHC-HL run, a production of up to $\mathcal{O}(10^7)$ pairs is likely to not be excluded by LHC Higgs searches, and new physics can be tested if ${\cal G}_h \tilde{f}'_\tau \gtrsim 10^{-7}$. This production channel appears suppressed as compared to production from $B$ meson decays, but the geometric factor ${\cal G}_h$ and $\tilde{f}'_\tau$ are different in both cases. The produced Higgs is much less boosted than the $B$ mesons such that the $\phi$ angular distribution is almost spherical, such that (with the currently planned geometry)  ${\cal G}_h\sim XXX$ \MM{DC this requires your attention.}. \DC{this is all identical to SM+S discussion... I'm not sure exactly what $G_h$ is, but from our generic signal studies in section 3, it's not gonna be hugely different from B decays}Furthermore, the relaxions (and therefore also the resulting $XX$ pairs) are more strongly boosted.  The probability of having $X$ decaying in the detector is 
\be
\tilde{f}'_\tau < \exp\left(\frac{-l}{\gamma \beta c \tau_X} \right)-\exp\left(-\frac{l+20/\sin \vartheta}{\gamma \beta c \tau_X}\right),
\ee
still with  $\sin \vartheta=0.32$, but now with a boost factor $\gamma \beta=|p_\phi|/ m_\phi$ where, $|p_\phi| \sim (m_h - 2 m_\phi) / 2$. 
Furthermore, the $B\rightarrow K \phi$ channel can only constrain $m_\phi\lesssim 4$~GeV, where the decay to the relaxion is kinematically allowed, while the  $h\rightarrow \phi\phi$ channel applies also at higher masses.\MM{I don't understand what the punchline is.}


\DC{all the details are pretty much irrelevant, just SM+S rehash. the POINT seems to be that relaxions motivate SM+S models where the S decays to LLPs. So we should do something similar to how the corresponding scenario is discussed for the dark photon (where the dark photon can be a source of LLP dark hadrons): 1) discuss more about the theory motivation for the relaxion decaying to LLPs, 2) just show relaxion production cross-section as function of relaxion mass, for some fixed mixing angle. (Pretty simple, just B and H decays). Then using arguments from section 3, whenever that production xsec is above 1fb, you could see LLps for some range of lifetimes. It'll make the section ~ 1 page. which is fine. }

\subsubsection{Conclusions}
We estimated the relaxion production from rare meson and Higgs decays and relaxion decays into SM particles or BSM ultra-long-lived particles.
In order for the relaxion to be sufficiently produced \textit{and} sufficiently long-lived within the sensitivity of MATHUSLA, we conclude that it must be either lighter than a GeV or it must decay into new ultra-long-lived particles.


==> tmp <==
\author{
Editors: \\
R.~Contino$^{1,2}$,\, 
D.~Curtin$^{3}$,\,
A.~Katz$^{1,4}$,\,
M.~L.~Mangano$^{1}$,\,
G.~Panico$^{5}$,\,
M.~J.~Ramsey-Musolf$^{6,7}$,\, 
G.~Zanderighi$^{1}$\,
\\
Contributors: \\
C.~Anastasiou$^{8}$,\,
W.~Astill$^{9}$,\,
J.~K.~Behr$^{10,11}$,\,
W.~Bizon$^{9}$,\,
P.~S.~Bhupal~Dev$^{12}$,\,
D.~Bortoletto$^{10}$,\,
F.~Caola$^{1}$,\,
J.~Chakrabortty$^{13}$,\,
C.-Y.~Chen$^{14,15,16}$,\,
F.~Dulat$^{8}$,\,
G.~Bambhaniya$^{17}$,\,
D.~Buttazzo$^{18}$
D.~de~Florian$^{19}$,\,
C.~Englert$^{20}$,\,
J.~A.~Frost$^{10}$,\,
B.~Fuks$^{21}$,\,
T.~Gherghetta$^{22}$,\,
G.~Giudice$^{1}$,\,
J.~Gluza$^{23}$,\,
N.~Greiner$^{24}$,\,
H.~Gray$^{25}$,\,
N.~P.~Hartland$^{10}$,\,
C.~Issever$^{10}$,\,
T.~Jeli\'nski$^{23}$,\,
A.~Karlberg$^{9}$,\,
J.~H.~Kim,$^{26,27,28}$,\,
F.~Kling$^{29}$,\,
A.~Lazopoulos$^{8}$,\,
S.~J.~Lee$^{30,31}$,\,
G.~Luisoni$^{1}$,\,
J.~Mazzitelli$^{19,32}$,\,
B.~Mistlberger$^{1}$,\,
P.~Monni$^{9}$,\,
K.~Nikolopoulos$^{33}$,\,
R.~N~Mohapatra$^{3}$,\,
A.~Papaefstathiou$^{1}$,\,
M.~Perelstein$^{34}$,\,
F.~Petriello$^{35}$,\,
T.~Plehn$^{36}$,\,
P.~Reimitz$^{36}$,\,
J.~Ren$^{37}$,\,
J.~Rojo$^{10}$,\,
K.~Sakurai$^{38}$,\,
T.~Schell$^{36}$,\,
F.~Sala$^{39}$,\,
M.~Selvaggi$^{40}$,\,
H.-S.~Shao$^{1}$,\,
M.~Son$^{26}$,\,
M.~Spannowsky$^{38}$,\,
T. Srivastava$^{13}$,\,
S.-F.~Su$^{29}$,\,
R. Szafron$^{41}$,\,
T.~Tait$^{42}$,\,
A.~Tesi$^{43}$,\,
A.~Thamm$^{44}$,\,
P.~Torrielli$^{45}$,\,
F.~Tramontano$^{46}$,\,
J.~Winter$^{47}$,\,
A.~Wulzer$^{48}$,\,
Q.-S.~Yan$^{49,50,51}$,\,
W.~M.~Yao$^{52}$,\,
Y.-C.~Zhang$^{53}$,\,
X.~Zhao$^{49}$,\,
Z.~Zhao$^{49,54}$,\,
Y.-M.~Zhong$^{55}$,\, 
Q.-H.~Cao$^{50,56,57}$,\, 
S.-L.~Chen$^{50,58}$,\, 
Y.~Liu$^{56}$
\vspace*{2cm}
}

\institute{
$^{1}$ CERN, TH Department, CH-1211 Geneva, Switzerland. \\
$^{2}$ EPFL, Lausanne, Switzerland. \\
$^{3}$Maryland Center for Fundamental Physics, Department of Physics, University of Maryland, College
Park, MD 20742, USA\\
$^{4}$Universit\'{e} de Gen\`{e}ve, Department of Theoretical Physics and Center for Astroparticle Physics,
24 quai E. Ansermet, CH-1211, Geneva 4, Switzerland\\
$^{5}$ IFAE, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Barcelona\\
$^{6}$ Amherst Center for Fundamental Interactions, Physics Department,University of Massachusetts Amherst, Amherst, MA 01003, USA\\
$^{7}$ Kellogg Radiation Laboratory, California Institute of Technology, Pasadena, CA 91125 USA\\
$^{8}$  Institute for Theoretical Physics, ETH Z\"urich,  8093 Z\"urich, Switzerland \\
$^{9}$ Rudolf Peierls Centre for Theoretical Physics, 1 Keble Road, University of Oxford, UK \\
$^{10}$ Physics Department, 1 Keble Road, University of Oxford, United Kingdom\\
$^{11}$ Deutsches Elektronen-Synchrotron (DESY), Notkestrasse 85, D-22607 Hamburg, Germany\\
$^{12}$Max-Planck-Institut f\"ur Kernphysik, Saupfercheckweg 1,
D-69117 Heidelberg, Germany\\
$^{13}$  Department of Physics, Indian Institute of Technology, Kanpur-208016, India\\
$^{14}$ Department of Physics, Brookhaven National Laboratory, Upton, New York 11973, USA\\
$^{15}$ Department of Physics and Astronomy, University of Victoria, Victoria, British Columbia V8P 5C2, Canada\\
$^{16}$ Perimeter Institute for Theoretical Physics, Waterloo, Ontario N2J 2W9, Canada\\
$^{17}$ Theoretical Physics Division, Physical Research Laboratory, Ahmedabad-380009, India\\
$^{18}$ Physik-Institut, Universit\"at Z\"urich, CH-8057 Z\"urich, Switzerland \\ 
$^{19}$ International Center for Advanced Studies (ICAS), UNSAM, Campus Miguelete, 25 de Mayo y Francia, (1650) Buenos Aires, Argentina\\
$^{20}$ SUPA, School of Physics and Astronomy, University of Glasgow,
Glasgow G12 8QQ, UK \\
$^{21}$ Sorbonne Universit\'es, UPMC Univ.~Paris 06, UMR 7589, LPTHE, F-75005 Paris, France.  CNRS, UMR 7589, LPTHE, F-75005 Paris, France \\
$^{22}$ School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA\\
 $^{23}$ Institute of Physics, University of Silesia, Uniwersytecka 4, 40-007 Katowice, Poland\\
$^{24}$ Physik Institut, Universit\"at Z\"urich, Winterthurerstrasse 190, CH-8057 Z\"urich, Switzerland \\
$^{25}$ CERN, EP Department, CH-1211 Geneva, Switzerland. \\
$^{26}$ Department of Physics, Korea Advanced Institute of Science and Technology, 335 Gwahak-ro, Yuseong-gu, Daejeon 305-701, Korea \\
$^{27}$ Center for Theoretical Physics of the Universe, IBS, 34051 Daejeon, Korea\\
$^{28}$ Center for Axion and Precision Physics Research, IBS, 34141 Daejeon, Korea \\
$^{29}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{30}$ Department of Physics, Korea University, Seoul 136-713, Korea\\
$^{31}$ School of Physics, Korea Institute for Advanced Study, Seoul 130-722, Korea\\
$^{32}$ Departamento de Fisica and IFIBA, FCEyN, Universidad de
Buenos Aires, (1428) Pabellon 1 Ciudad Universitaria, Capital Federal,
Argentina \\
$^{33}$ School of Physics and Astronomy, University of Birmingham,
Birmingham, B15 2TT, United Kingdom \\
$^{34}$Laboratory for Elementary Particle Physics, Cornell University,
Ithaca, NY 14853, USA\\
$^{35}$ 
Northwestern University, Department of Physics and Astronomy, 2145
Sheridan Road, 
Evanston, Illinois 60208-3112, USA\\
$^{36}$ Institut f\"ur Theoretische Physik, Universit\"at Heidelberg, Germany \\
$^{37}$ Department of Physics, University of Toronto, Toronto, Ontario, Canada M5S1A7\\
$^{38}$ IPPP, Department of Physics, University of Durham, Science Laboratories, South Road, Durham, DH1 3LE, UK\\
$^{39}$ 2LPTHE, CNRS, UMR 7589, 4 Place Jussieu, F-75252, Paris, France\\
$^{40}$ Centre for Cosmology, Particle Physics and Phenomenology CP3, Universit\'e Catholique de Louvain, Chemin du Cyclotron, 1348 Louvain la Neuve, Belgium\\
$^{41}$ Department of Physics, University of Alberta, Edmonton, AB
T6G 2E1, Canada\\
$^{42}$ Department of Physics and Astronomy, University of California, Irvine, CA 92697, USA\\
$^{43}$ Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA\\
$^{44}$ PRISMA Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany\\
$^{45}$ Dipartimento di Fisica, Universit\`a di Torino, and INFN, Sezione di Torino, \\
Via P.~Giuria~1, I-10125, Turin, Italy \\
$^{46}$ Universit\`a di Napoli ``Federico II'' and INFN, Sezione di
Napoli, 80126 Napoli, Italy \\
$^{47}$Department of Physics and Astronomy, Michigan State University,
East Lansing, MI 48824, USA\\
$^{48}$Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova and
INFN, Sezione di Padova, via Marzolo 8, I-35131 Padova, Italy\\
$^{49}$ School of Physical Sciences, University of Chinese Academy of Sciences, Beijing 100049, P. R. China\\
$^{50}$ Center for High-Energy Physics, Peking University, Beijing 100871, P. R. China\\
$^{51}$ Center for future high energy physics, Chinese Academy of Sciences 100049, P. R. China\\
$^{52}$ Lawrence Berkeley National Lab (LBNL), One Cyclotron Rd, Berkeley, CA94720, USA\\
$^{53}$ Service de Physique Th\'eorique, Universit\'e Libre de Bruxelles, Boulevard du Triomphe, CP225, 1050 Brussels, Belgium\\
$^{54}$ Department of Physics, University of Siegen, 57068 Siegen, Germany\\
$^{55}$ C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, New York 11794, USA\\
$^{56}${Department of Physics and State Key Laboratory of Nuclear
Physics and Technology, Peking University, Beijing 100871, China} \\
$^{57}${Collaborative Innovation Center of Quantum Matter,
Beijing 100871, China} \\
$^{58}${Key Laboratory of Quark and Lepton Physics (MoE) and Institute of
Particle Physics, Central China Normal University, Wuhan 430079,
China} \\

}

